Temporal Treasure Hunt: Content-based Time Series Retrieval System for Discovering Insights

Time series data is ubiquitous across various domains such as finance, healthcare, and manufacturing, but their properties can vary significantly depending on the domain they originate from. The ability to perform Content-based Time Series Retrieval (CTSR) is crucial for identifying unknown time series examples. However, existing CTSR works typically focus on retrieving time series from a single domain database, which can be inadequate if the user does not know the source of the query time series. This limitation motivates us to investigate the CTSR problem in a scenario where the database contains time series from multiple domains. To facilitate this investigation, we introduce a CTSR benchmark dataset that comprises time series data from a variety of domains, such as motion, power demand, and traffic. This dataset is sourced from a publicly available time series classification dataset archive, making it easily accessible to researchers in the field. We compare several popular methods for modeling and retrieving time series data using this benchmark dataset. Additionally, we propose a novel distance learning model that outperforms the existing methods. Overall, our study highlights the importance of addressing the CTSR problem across multiple domains and provides a useful benchmark dataset for future research.

==> insert/alg_dtw.tex <==
\begin{algorithm}[ht]
    \centering
    \caption{DTW Distance\label{alg:dtw}}
    % \footnotesize
    \begin{algorithmic}[1]
        \Input{time series~$\mathbf{a} \in \mathbb{R}^w$, time series~$\mathbf{b} \in \mathbb{R}^h$}
        \Function{DTW}{$\mathbf{a}, \mathbf{b}$}
        \State $D \gets $ zero matrix $\in \mathbb{R}^{w \times h}$
        \For{$i$ \textbf{in} $[0, \cdots, w)$}
        \For{$j$ \textbf{in} $[0, \cdots, h)$}
        \State $D[i, j] \gets |a[i] - b[j]|$
        \EndFor
        \EndFor
        \For{$i$ \textbf{in} $[0, \cdots, w)$}
        \For{$j$ \textbf{in} $[0, \cdots, h)$}
        \State $D[i,j] \gets D[i,j] + \textsc{min}(D[i-1, j],D[i, j-1],D[i-1, j-1])$
        \EndFor
        \EndFor
        \State \Return $D[w-1, h-1]$
        \EndFunction
    \end{algorithmic}
\end{algorithm}


==> insert/fig_cd_diag.tex <==
\begin{figure}[ht]
\centerline{
\includegraphics[width=0.99\linewidth]{insert/figure/fig_cd_ndcg10_0.pdf}
}
\caption{
The proposed method is statistically significantly better than the others based on the critical difference (CD) diagram.
We also construct the CD diagram for PREC@10 and PR@10, the conclusion remains the same.
}
\label{fig:cd_diag}
\end{figure}

==> insert/fig_nonmetric.tex <==
\begin{figure}[ht]
\centerline{
\includegraphics[width=0.6\linewidth]{insert/figure/fig_nonmetric_1.pdf}
}
\caption{
Human similarity judgment is often non-metric.
}
\label{fig:nonmetric}
\end{figure}
